Snowy: Recommending Utterances for Conversational Visual Analysis

Natural language interfaces (NLIs) have become a prevalent medium for conducting visual data analysis, enabling people with varying levels of analytic experience to ask questions of and interact with their data. While there have been notable improvements with respect to language understanding capabilities in these systems, fundamental user experience and interaction challenges including the lack of analytic guidance (i.e., knowing what aspects of the data to consider) and discoverability of natural language input (i.e., knowing how to phrase input utterances) persist. To address these challenges, we investigate utterance recommendations that contextually provide analytic guidance by suggesting data features (e.g., attributes, values, trends) while implicitly making users aware of the types of phrasings that an NLI supports. We present SNOWY, a prototype system that generates and recommends utterances for visual analysis based on a combination of data interestingness metrics and language pragmatics. Through a preliminary user study, we found that utterance recommendations in SNOWY support conversational visual analysis by guiding the participants' analytic workflows and making them aware of the system's language interpretation capabilities. Based on the feedback and observations from the study, we discuss potential implications and considerations for incorporating recommendations in future NLIs for visual analysis.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> listings-and-more/CIM-example.tex <==

\begin{dialogue}
    \speak{Tintin}  \indent \hspace{3mm} What is trend of worldwide gross over the years? $C_f=\{ \textrm{Worldwide Gross, Release Years} \}$
    \speak{\snowy} \direct{Infers a trend intent and creates a line chart showing average gross over time.}
    \speak{Tintin}  \indent \hspace{4mm} show me the orange spike. \textbf{CONTINUE}
    \\ \indent \hspace{7mm} $C_b=\{ \textrm{measles, uk} \}$, $C_f=\{ \textrm{measles, uk, orange spike} \}$
    \speak{\snowy} \direct{Highlights spike in the line for measles in the line chart.}
    \speak{Tintin}  \indent \hspace{4mm} mumps over there.
      \\ \indent \hspace{7mm} \textbf{RETAIN} $C_b=\{ \textrm{uk} \}$, $C_f=\{ \textrm{uk} \}$
     \\ \indent \hspace{7mm} \textbf{SHIFT} $C_b=\{ \textrm{measles, orange spike} \}$, $C_f=\{ \textrm{mumps} \}$
     \speak{\snowy} \direct{Retains spatial filter for UK, updates categorical filter to
     \\ \indent \hspace{7mm}  mumps, removes highlighted spike in the line for measles.}
    \speak{Tintin}  \indent \hspace{4mm} measles epidemic in malawi congo angola.
      \\ \indent \hspace{7mm} \textbf{SHIFT} $C_b=\{ \textrm{mumps} \}$, $C_f=\{ \textrm{measles, epidemic} \}$
     \\ \indent \hspace{7mm} \textbf{SHIFT} $C_b=\{ \textrm{uk} \}$, $C_f=\{ \textrm{malawi, congo, angola} \}$
     \speak{\snowy} \direct{Applies categorical filter for measles epidemics, applies new
        \\ \indent \hspace{7mm} spatial filter on Malawi, Congo, and Angola, replacing UK.}
\end{dialogue}



==> listings-and-more/context-state-changes.tex <==
\begin{figure}[t!]
\begin{minipage}[t]{0.33\textwidth}
\centering
\begin{minted}
[
baselinestretch=1,
fontsize=\scriptsize,
breaklines,
escapeinside=@@,
style=manni
]{javascript}
"utterance": "",
"vis":{},
"selection":[],
"interactionScores": {
  "attributes": [
    Content Rating: 0
    Worldwide Gross: 0,
    Production Budget: 0,
    Release Year: 0,
    ...
  ],
  "intents": [
    distribution: 0,
    group: 0,
    correlation: 0,
    trend: 0,
    filter: 0,
    aggregation: 0
  ],
  ...
}
@\newline\newline@
\end{minted}
(A)
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\centering
\begin{minted}
[
baselinestretch=1,
fontsize=\scriptsize,
breaklines,
escapeinside=@@,
style=manni
]{javascript}
"utterance": "Compare across Content Ratings",
"vis":{
    mark: "line",
    encoding: {x: "Release Year",...}
},
"selection":[],
"interactionScores": {
  "attributes": [
    Content Rating: 1,
    Worldwide Gross: 1,
    Release Year: 1,
    Production Budget: 0
    ...
  ],
  "intents": [
    trend: 1,
    group: 1,
    distribution: 0,
    correlation: 0,
    filter: 0,
    aggregation: 0
  ],
  ...
}
\end{minted}
(B)
\end{minipage}
\begin{minipage}[t]{0.33\textwidth}
\centering
\begin{minted}
[
baselinestretch=1,
fontsize=\scriptsize,
breaklines,
escapeinside=@@,
style=manni
]{javascript}
"utterance": "Break down by Creative Types",
"vis":{
    mark: "point",
    encoding: {x: "Production Budget",...}
},
"selection":[{...},{...},...],
"interactionScores": {
  "attributes": [
    Worldwide Gross: 3,
    Production Budget: 2
    Content Rating: 2,
    IMDB Rating: 1,
    ...
  ],
  "intents": [
    group: 3,
    trend: 2,
    filter: 2,
    correlation: 1,
    distribution: 0,
    aggregation: 0
  ],
  ...
}
\end{minted}
(C)
\end{minipage}
\caption{Updates to the context state object maintained by \snowy~during Tintin's exploration of the movies dataset.
States shown are passed as input to the recommendation engine to get utterances at different points during the usage scenario.
With respect to the scenario described in Section~\ref{sec:interface-and-scenario}, (A) maps to Figure~\ref{fig:teaser}A, (B) maps to Figure~\ref{fig:scenario-1}A, and (C) shows the context state object during the deictic action of selecting points towards the end of the scenario shown in Figure~\ref{fig:teaser}C.\arjun{make this more graphical. Try to have fewer states if needed but highlight changes}}
\label{fig:context-state-changes}
\end{figure}

==> listings-and-more/context-state-object.tex <==
\begin{listing}
\begin{minted}[frame=none,
               linenos=false,
               xleftmargin=21pt,
               tabsize=4]{js}
{     
    "activeUtterance": "Show average Worldwide Gross by Major Genre",
    "activeVis":{x:genre,y:avg(gross),mark:bar},
    "activeSelection":[],
    "interestMap": {}
}
\end{minted}
\caption{Context state object in \snowy. \vidya{Need a text version of the interest map. What I got was a screenshot.}}
\label{fig:contesxt-state-object}
\end{listing}

==> listings-and-more/reco-algo-main.tex <==
% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{algorithm}[H]%<-- Remove float environment
% \SetAlgoLined
% % \KwData{contextState}
% % \KwResult{Recommendations}
%  recos = []\\
%     \uIf{hasActiveSelections(contextState)}{
%         recos.add(getDeicticRecos(contextState))
%     }
%     \uElse{
%         \uIf{hasActiveChart(contextState)==false}{
%             recos.add(getNewInquiryRecos(contextState))
%         }
%         \uElse{
%             recos.add(getFollowUpRecos(contextState))\\
%             recos.add(getNewInquiryRecos(contextState))
%         }
%     }~\\
 
%  populateRecommendationObjects(recos)\\
 
%  \textbf{return} recos
 
% \caption{getRecommendations(contextState)}
% \label{algo:get-recos}
% \end{algorithm}
% \end{wrapfigure}

\begin{wrapfigure}{r}{0cm}
\begin{minipage}{.6\textwidth}
\centering
\begin{minted}
[
baselinestretch=1,
frame=lines,
fontsize=\small,
% linenos,
% xleftmargin=15pt,
breaklines,
% style=manni,
style=vs,
escapeinside=@@
]{text}

@{\normalsize{{\textbf{Algorithm:} Generating utterance recommendations}}}
\textbf{Input}: Interface context state (\variable{contextState})
\textbf{Output}: Recommendations (\variable{recos})@

1. If there are active mark selections in the @\variable{contextState}@, add deictic utterance recommendations to @\variable{recos}@ and go to step 4. Else, go to step 2.

2. If there is no active chart in the @\variable{contextState}@, skip to step 3. Else, add follow-up utterance recommendations to @\variable{recos}@ and then go to step 3.

3. Add utterance recommendations for new inquiries to @\variable{recos}@.

4. Return @\variable{recos}@.
\end{minted}
\label{algo:get-recos}
\captionof{listing}{Pseudocode summarizing logic used to select recommendation types to show given a context state object.}
\end{minipage}
\end{wrapfigure}

==> listings-and-more/reco-algo-populate.tex <==
\begin{wrapfigure}{r}{0cm}
\begin{minipage}{.6\textwidth}
\centering
\begin{minted}
[
baselinestretch=1,
frame=lines,
fontsize=\small,
% linenos,
% xleftmargin=15pt,
breaklines,
style=vs,
escapeinside=@@
]{python}

def populateRecommendations(recos,contextState):
  for reco in recos:
    recoTemplate = getTemplate(reco,contextState) # selects a template based on the recommendation type. When available, both the active view and the language of the active utterance are also considered when selecting templates
    if reco.subType == 'shift-trend':
      attrPairs = getAttrPairs_trend('stddev+interaction',contextState) # gets a list of (@\texttt{T}@x@\texttt{Q}@) attribute pairs ordered based on standard deviation in the underlying data and the contextState.interactionScores
      realizeUtterance(recoTemplate,contextState,@\newline@{'dimensions':[attrPairs[0]['dimension']],@\newline@'measures':[attrPairs[0]['measure']]})
    else if reco.subType == 'shift-correlation':
      attrPairs = getAttrPairs_corr('pearson+interaction',contextState) # gets a list of (@\texttt{Q}@x@\texttt{Q}@) attribute pairs ordered based on the Pearson's correlation coefficients and the contextState.interactionScores
      realizeUtterance(recoTemplate,contextState,@\newline@{'measures':attrPairs[0]})
    @{\vdots}@
    else if reco.subType == 'continue-filter':
      if contextState.visType == 'bar_chart':
        filterAttr = getDimensionAttr(contextState.vis)
        filterVals = getTopNFilters(contextState.vis,filterAttr,3) # returns a list of filter values for the given attribute in the context of the active visualization
        realizeUtterance(recoTemplate,contextState,@\newline@{'filterAttrs':[filterAttr],'filterVals':filterVals}}
      @{\vdots}@
\end{minted}
\label{algo:populate-reco}
\captionof{listing}{Pseudocode summarizing logic used to parameterize and linguistically realize filtered recommendation objects.}
\end{minipage}
\end{wrapfigure}

==> listings-and-more/reco-algos-individual-code.tex <==
\begin{wrapfigure}{r}{0cm}
\begin{minipage}{.575\textwidth}
\centering
\begin{minted}
[
baselinestretch=1,
frame=lines,
fontsize=\small,
% linenos,
% xleftmargin=15pt,
breaklines,
% style=manni,
style=vs,
escapeinside=@@
]{python}

def getDeicticRecommendations(contextState):
  recos = []
  if contextState.visType == "scatterplot":
    if contextState.selections.length > 1: # if there are multiple points selected, suggest utterances for performing popular calculations for the active chart type
      recos.add(getRecoObj('compute-aggregate'))
      recos.add(getRecoObj('compute-correlation'))
  @{\large{\vdots}}@
  rankRecommendations(recos,contextState,'intent','min')
  return recos
\end{minted}
\begin{minted}
[
baselinestretch=1,
frame=lines,
fontsize=\small,
% linenos,
% xleftmargin=15pt,
breaklines,
% style=manni,
style=vs,
escapeinside=@@
]{python}

def getFollowUpRecommendations(contextState):
  recos = []
  if hasFreeEncodingChannels(contextState.vis):
    recos.add(getRecoObj('continue',contextState) # based on the attribute types and available encodings in contextState.vis, select one of 'continue-correlation', 'continue-group', 'continue-aggregation', or 'continue-trend'
  if isAggregated(contextState.vis):
    recos.add(getRecoObj('shift-aggregation',contextState)) # inspect the aggregation function in contextState.vis and contextState.utterance (if available) to suggest switching to other aggregation functions
  
  recos.add(getRecoObj('filter',contextState)) # inspect the attributes and filters in contextState.vis to suggest new filters ('continue-filter') or adjust current filters ('shift-filter')
  
  rankRecommendations(recos,contextState,'intent','min')
  return recos
\end{minted}
\begin{minted}
[
baselinestretch=1,
frame=lines,
fontsize=\small,
% linenos,
% xleftmargin=15pt,
breaklines,
% style=manni,
style=vs,
escapeinside=@@
]{python}

def getNewInquiryRecommendations(contextState):
  recos = []
  for recoSubType in ['shift-distribution','shift-group','shift-correlation',@\newline@'shift-trend']:
    recos.add(getRecoObj(recoSubType,contextState)) # generate utterances for new inquiries by referring to the active view and utterance from the contextState
  
  rankRecommendations(recos,contextState,'intent','min')
  return recos
\end{minted}
\label{algo:get-recos-individual}
\captionof{listing}{Pseudocode summarizing logic for filtering and ranking different types of utterance recommendations.}
\end{minipage}
\end{wrapfigure}

% \begin{wrapfigure}{r}{0.55\textwidth}
% \begin{algorithm}[H]%<-- Remove float environment
% \SetAlgoLined
% % \KwData{contextState}
% % \KwResult{Recommendations}
%  recos = []\\
%     \uIf{contextState.visType=="scatterplot"}{
%         \uIf{contextState.selection.length>1}{
%             recos.add(getRecoObj(`compute-aggregate'))\\
%             recos.add(getRecoObj(`compute-correlation'))
%         }
%     }
%     \vdots
 
%  \textbf{return} recos
 
% \caption{getDeicticRecos(contextState)}
% \label{algo:get-deictic-recos}
% \end{algorithm}

% \begin{algorithm}[H]%<-- Remove float environment
% \SetAlgoLined
% % \KwData{contextState}
% % \KwResult{Recommendations}
%  recos = []\\
%  vis = contextState.activeVisSpec\\
 
%  \uIf{hasFreeEncodings(vis)}{
%     recos.add(getRecoObj(``continue'',contextState))~\algocomment{//checks active attributes and available encoding channels to suggest one of `continue-group', `continue-aggregation', `continue-correlation', or `continue-trend'}
%  }
 
%  \textbf{return} recommendations
 
% \caption{getFollowUpRecos(contextState)}
% \label{algo:get-followup-recos}
% \end{algorithm}

% \begin{algorithm}[H]%<-- Remove float environment
% \SetAlgoLined
% % \KwData{contextState}
% % \KwResult{Recommendations}
%  recommendations = []\\
%     \uIf{hasActiveSelections(contextState)}{
%         recommendations.add(getDeicticRecommendations(contextState))
%     }
%     \uElse{
%         \uIf{hasActiveChart(contextState)==false}{
%             recommendations.add(getNewInquiryRecommendations(contextState))
%         }
%         \uElse{
%             recommendations.add(getFollowUpRecommendations(contextState))\\
%             recommendations.add(getNewInquiryRecommendations(contextState))
%         }
%     }~\\
 
%  populateRecommendationObjects(recommendations)\\
 
%  \textbf{return} recommendations
 
% \caption{getRecommendations(contextState)}
% \label{algo:get-new-inquiry-recos}
% \end{algorithm}
% \end{wrapfigure}

==> listings-and-more/reco-algos-individual.tex <==
\begin{wrapfigure}{r}{0cm}
\begin{minipage}{.575\textwidth}
\centering
\begin{minted}
[
baselinestretch=1,
frame=lines,
fontsize=\footnotesize,
breaklines,
style=vs,
escapeinside=@@
]{text}

@{\small{{\textbf{Algorithm:} Generating deictic recommendations}}}
\textbf{Input}: Interface context state (\variable{contextState})
\textbf{Output}: Recommendations (\variable{recos})@

1. Check the current chart type in @\variable{contextState}@ to identify which computational functions are supported (e.g., calculating averages and correlation coefficients in scatterplots).

2. For each supported function, check if the active selection in the @\variable{contextState}@ meets the function criteria (e.g., at least two data items are needed for computing differences) and add corresponding utterance to @\variable{recos}@.

3. Return @\variable{recos}@.

\end{minted}
\begin{minted}
[
baselinestretch=1,
frame=lines,
fontsize=\footnotesize,
% linenos,
% xleftmargin=15pt,
breaklines,
% style=manni,
style=vs,
escapeinside=@@
]{text}

@{\small{{\textbf{Algorithm:} Generating follow-up recommendations}}}
\textbf{Input}: Interface context state (\variable{contextState})
\textbf{Output}: Recommendations (\variable{recos})@

\end{minted}
\begin{minted}
[
baselinestretch=1,
frame=lines,
fontsize=\small,
% linenos,
% xleftmargin=15pt,
breaklines,
% style=manni,
style=vs,
escapeinside=@@
]{python}

def getNewInquiryRecommendations(contextState):
  recos = []
  for recoSubType in ['shift-distribution','shift-group','shift-correlation',@\newline@'shift-trend']:
    recos.add(getRecoObj(recoSubType,contextState)) # generate utterances for new inquiries by referring to the active view and utterance from the contextState
  
  rankRecommendations(recos,contextState,'intent','min')
  return recos
\end{minted}
\label{algo:get-recos-individual}
\captionof{listing}{Pseudocode summarizing logic for filtering and ranking different types of utterance recommendations.}
\end{minipage}
\end{wrapfigure}

% \begin{wrapfigure}{r}{0.55\textwidth}
% \begin{algorithm}[H]%<-- Remove float environment
% \SetAlgoLined
% % \KwData{contextState}
% % \KwResult{Recommendations}
%  recos = []\\
%     \uIf{contextState.visType=="scatterplot"}{
%         \uIf{contextState.selection.length>1}{
%             recos.add(getRecoObj(`compute-aggregate'))\\
%             recos.add(getRecoObj(`compute-correlation'))
%         }
%     }
%     \vdots
 
%  \textbf{return} recos
 
% \caption{getDeicticRecos(contextState)}
% \label{algo:get-deictic-recos}
% \end{algorithm}

% \begin{algorithm}[H]%<-- Remove float environment
% \SetAlgoLined
% % \KwData{contextState}
% % \KwResult{Recommendations}
%  recos = []\\
%  vis = contextState.activeVisSpec\\
 
%  \uIf{hasFreeEncodings(vis)}{
%     recos.add(getRecoObj(``continue'',contextState))~\algocomment{//checks active attributes and available encoding channels to suggest one of `continue-group', `continue-aggregation', `continue-correlation', or `continue-trend'}
%  }
 
%  \textbf{return} recommendations
 
% \caption{getFollowUpRecos(contextState)}
% \label{algo:get-followup-recos}
% \end{algorithm}

% \begin{algorithm}[H]%<-- Remove float environment
% \SetAlgoLined
% % \KwData{contextState}
% % \KwResult{Recommendations}
%  recommendations = []\\
%     \uIf{hasActiveSelections(contextState)}{
%         recommendations.add(getDeicticRecommendations(contextState))
%     }
%     \uElse{
%         \uIf{hasActiveChart(contextState)==false}{
%             recommendations.add(getNewInquiryRecommendations(contextState))
%         }
%         \uElse{
%             recommendations.add(getFollowUpRecommendations(contextState))\\
%             recommendations.add(getNewInquiryRecommendations(contextState))
%         }
%     }~\\
 
%  populateRecommendationObjects(recommendations)\\
 
%  \textbf{return} recommendations
 
% \caption{getRecommendations(contextState)}
% \label{algo:get-new-inquiry-recos}
% \end{algorithm}
% \end{wrapfigure}

==> sections/datachat.tex <==
\section{DataChat}

\begin{itemize}
    \item To show other applications of utterance recommendations and Snowy's generalizability, we incorporate it in a second prototype, DataChat---a mobile visualization system.
    \item Show some screenshots with a different dataset (ideally personal health, travel, finance, or covid related) and describe them. May not need to give a full scenario walkthrough.
\end{itemize}

==> sections/discussion.tex <==
\section{Discussion}

\begin{itemize}
    \item Predictability of recos. (interesting point about a separate undo stack for recommendations in P11's session)
    \item Over-reliance on recos.
\end{itemize}

==> sections/old/intro.tex <==
The increase in popularity of NLI tools for visual analysis is due to the fact that they
do not require users to learn the nuances of a complex tool, or employ complex query languages
such as SQL, or understand the exact schema of the data.
Recent advances in natural language processing and machine learning have resulted in considerable improvements in NLIs for understanding a range of query intents~\cite{datatone,eviza,hoque2017applying,srinivasan2018orko,askdata,thoughtspot,powerbi,ibmwatson}.
The vocabulary and parsing capabilities supported in such systems enable users to explore complex analytical questions beyond simple keyword queries.

Despite improvements in query understanding, formulating utterances during an analytical flow can be challenging to the user for several reasons. First, analytical query formulation involves the need to understand the characteristics of the underlying data and the various domains included in the dataset (e.g., range, level of detail of the attributes)~\cite{sneakpique}. Second, 
ambiguity and underspecification are prevalent in language and users may often need to repair or refine their utterances to match their mental model to that of the computer~\cite{Setlur:IUI}. Third, exploratory visual analysis is an iterative process of
asking and answering questions about data through visualizations where new questions often arise from unexpected
observations. Users need to understand whether they are finding new insights and a lack of guidance can interfere with an accurate sense of progress towards their analytical goal~\cite{grammel2010information,zenvisage}. While visualization recommendation (VisRec) systems guide users along their
exploration journey by suggesting effective visual encodings~\cite{Mackinlay:2007,Wongsuphasawat2016,Wongsuphasawat2017} or potentially interesting visualizations~\cite{datasite,hu2018dive,Vartak2015,wills2010autovis,demiralp2017foresight,seo2005rank}, they do not provide utterance recommendations that specifically guide the user in their analytical conversation with the system.


%% need to talk more about command-based interfaces here and elaborate on it.
\arjun{On the other hand, predefined command suggestions such as those in general NLIs (e.g., Alexa's weather command examples) may help familiarize users with the system's language but not offer contextual recommendations that assist visual data analysis...} These challenges pose additional cognitive load for users as they attempt to formulate natural language utterances based on the context of their analytical flow.

To address this problem, we developed a novel interface system called \snowy\footnote{The name Snowy is inspired by the namesake fictional dog in the \textit{Adventures of Tintin} comic series~\cite{tintin} where he addresses his internal monologue to the reader with speech bubbles. He can understand human language and his verbal responses to various situations include jokes, expressions of fright, and pleas to Tintin to exercise caution.}  that provides natural language utterances as recommendations during a user's visual analysis flow. These recommendations support both new inquiry and follow-up recommendations based on the user's current context by considering data interestingness as well as language pragmatics from the history of typed utterances.
Snowy is a mixed-initiative system that supports both natural language input and deictic interaction with the marks in the current visualization to suggest next-step utterances. 

\vidya{Now describe teaser}

Our contributions are summarized as follows:
\begin{itemize}
    \item Discuss a design space of utterance recommendations during visual data analysis.
    \item Present two systems, \sysnameA and \sysnameB, that operationalize the proposed utterance recommendations within a multimodal manual view specification interface and a conversational interface, respectively.
    \item Through an evaluation of \sysnameA, we highlight how utterance recommendations can guide visual analysis and improve discoverability/learnability in the context of NLIs for visualization.
\end{itemize}

==> sections/old/scenario.tex <==
\section{Motivating Scenario}
\label{sec:scenario}
\vidya{I am trying to understand the flow of having a description of using Snowy before the system is described. To me, a motivating scenario would be for example describing a user's analytical workflow in say a recommendations system or NLI and coming up with motivating design goals for how Snowy was realized.}
\arjun{Was trying to see if this can work as a way to bring in the ``demo" early in the paper. But I understand your concern and think we can go with the classic route of pushing this scenario to the start of the system section, making Design Considerations the new section 3.}
% \begin{itemize}
%     \item Use the current prototype to give a motivating example of what utterance recommendations could look like and how they can empower visual analysis.
%     \item Implicitly talk about system UI (no need to have another section about this).
% \end{itemize}

% Create a scenario that covers:
% - Using new inquiry recos
% - Using follow-up recos
% - Manual view specification and its effect on NL input
% - Using deictic recos
% - Using the "show more recos" option
% - at least 3 intents
% - linguistic variation for new inquiry (``Show Y over X'' vs.~``Now show Y instead'')

\begin{figure*}[b!]
    \centering
    \includegraphics[width=\textwidth]{figures/scenario/scenario-wide-zoomed-1.pdf}
    \caption{Exploring a movies dataset with \snowy. Sub-figure captions summarize the system state and actions.}
    \label{fig:scenario-1}
\end{figure*}

We first motivate \snowy's design and the idea of leveraging utterance recommendations for conversational visual analysis through a usage scenario (also illustrated in the supplementary video).
Consider Sarah, an analyst at a movie production house examining a dataset of previously released movies to identify the types of movies her company should invest in next.
The dataset contains 700 movies with nine attributes for each movie including its {\small{\faCalendar}}~\textit{Release Year}, {\small{\faFont}}~\textit{Major Genre}, {\small{\faHashtag}}~\textit{Worldwide Gross}, and {\small{\faHashtag}}~\textit{IMDB Rating}, among others (shown in Figure~\ref{fig:teaser}A).
For consistency, we use this movies dataset for examples throughout this paper.

As Sarah loads the dataset, \snowy~scans the underlying data to identify potentially interesting attribute combinations to explore and presents Sarah with a list of utterance suggestions she can use to start her exploration (Figure~\ref{fig:scenario-1}A).
Looking through the suggestions, Sarah finds the question of looking for trends in \textit{Worldwide Gross} over time relevant (\reco{What is the trend of \textbf{Worldwide Gross} over the \textbf{Release Years}?}) and clicks the recommendation to select it as her input utterance.
In response, \snowy~renders a line chart and then updates its recommendations to suggest new inquiries, while also including some suggestions of follow-up utterances to modify the active chart (Figure~\ref{fig:scenario-1}B).
Looking through the follow-up suggestions, Sarah gets intrigued by the idea of seeing changes over time across \textit{Content Ratings}, and selects one of the follow-up suggestions (\reco{Compare trends across \textbf{Content Ratings}}).
Through the updated multi-series line chart, Sarah notices that while all movie types except R-rated movies have a higher gross over time, PG-13 movies have had the most stable increase.
Sarah again looks through the new inquiries suggested by \snowy~and selects the recommendation \reco{Now show changes in \textbf{Production Budget} instead} to contrast trends across \textit{Worldwide Gross} and \textit{Production Budget}.
In response, \snowy~updates the line chart, swapping the \textit{Worldwide Gross} attribute on the Y-axis with the \textit{Production Budget}.
Through the updated chart, Sarah notices that movies follow a similar trend for the budget and correspondingly makes a note that her company should consider PG-13 movies more closely.

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figures/scenario/scenario-wide-zoomed-2.pdf}
    \caption{Exploring a movies dataset with \snowy~(cont'd). Sub-figure captions summarize the system state and actions.}
    \label{fig:scenario-2}
\end{figure*}

Wondering which attributes to explore next, Sarah skims the recommendations panel and stops when she sees the suggestion \reco{Show average \textbf{IMDB Rating} by \textbf{Major Genre}}.
She likes the idea of computing and comparing a derived value (in this case, average) for each genre but does not want to use the \textit{IMDB Rating}s.
To see alternative suggestions, she hovers on the recommendation and clicks the {\small{\faBars}} icon to see similar utterance recommendations (Figure~\ref{fig:scenario-1}D).
From the suggested list, she likes the idea of computing the average grosses across genres and selects \reco{Show average \textbf{Worldwide Gross} by \textbf{Major Genre}} as her input utterance.
Inspecting the resulting bar chart, Sarah observes that \textit{Action} and \textit{Adventure} have notably higher values.
In parallel, \snowy~also interprets the bar chart and recommends a series of follow-up suggestions, including one to drill down into the three highest grossing genres (\reco{Just show \textbf{Action, Adventure, and Musical}}).
As this matches her observation, Sarah selects this follow-up suggestion to refine the scope of her exploration and the system adds a \textit{Major Genre} filter, allowing Sarah to refine it further through the GUI if needed (Figure~\ref{fig:scenario-2}A).

Considering the active bar chart, Sarah's prior interactions, and the available data attributes, \snowy~now recommends two follow-up utterances to include \textit{Creative Type} as an additional attribute for comparison, or change the aggregation level of the current chart from \textit{average} to \textit{sum}.
\snowy~also infers that Sarah has performed analytic tasks like looking for trends over time and computed derived values for quantitative attributes over categorical ones.
Thus, to broaden her analytic coverage, \snowy~promotes utterances pertaining to other analytic tasks observing correlations between attributes and seeing the distribution items in the dataset in its new inquiry suggestions (Figure~\ref{fig:scenario-2}A-bottom right).
Furthermore, to promote data attribute coverage in her exploration, as part of its suggestions, \snowy~includes attributes that Sarah has not previously considered (e.g., \textit{Creative Type}, \textit{IMDB Rating}, \textit{Duration}).

Seeing the utterance \reco{Plot \textbf{IMDB Rating} versus \textbf{Rotten Tomatoes Rating}} at the top of the new inquiry suggestions, Sarah realizes that she has not considered movie ratings as part of her analysis so far and selects it as her input, resulting in \snowy~rendering a scatterplot comparing ratings across the two platforms (Figure~\ref{fig:scenario-2}B).
Sarah subsequently selects the follow-up suggestion \reco{Drill down into \textbf{PG-13}} to further filter down to \textit{PG-13} movies (since she had earlier noticed that these movies tend to have a stable return on investment over time).
Inspecting the scatterplot, Sarah confirms that there are no unexpected patterns and that the ratings across the IMDB and Rotten Tomatoes platforms are fairly correlated.
Thus, she decides to switch her focus back to the return on investment on movies and manually updates the scatterplot by dragging the \textit{Production Budget} and \textit{Worldwide Gross} attribute pills to the X- and Y-encoding shelves, respectively.
In response, \snowy~clears the text input box since the visualization was manually specified and updates its utterance suggestions based on the new chart (Figure~\ref{fig:scenario-2}C).
Sarah selects the follow-up suggestion \reco{Break down by \textbf{Creative Type}} since that is an attribute she had not previously considered, leading to the system coloring points by \textit{Creative Type}.

To inspect movies with a high gross and return on investment, Sarah draws a selection box on the chart around movies that gross over $~$500 million while having a budget of $~$200 million or below.
Through the active selection of 13 movies and the mark colors, Sarah identifies that \textit{Science Fiction} (five movies), \textit{Super Hero} (four movies) have the highest chance of success, with \textit{Contemporary Fiction} and \textit{Fantasy} (two movies each) also being creative types to consider.
Based on Sarah's active selection, \snowy~now suggests follow-up utterances for computations that can be performed on the selected items.
Sarah selects the suggestion \reco{What are the \textbf{average} values?} and notes that PG-13 movies having the specified genres and creative types gross, on average, 709 million on an average investment of 132 million.
She clears the view and continues exploring other aspects of the data to report any additional findings to her company's investment team.

==> sections/old/system.tex <==
\section{Snowy}

\begin{wrapfigure}{r}{0cm}
    \includegraphics[width=.6\linewidth,keepaspectratio]{figures/architecture.pdf}
    \caption{System architecture overview.\vidya{the font for ``snowy user interface'' looks too light and the UI screenshot next to it is too faint. Given how much space this figure is currently occupying, should it just span the entire width of the page?}}
    \label{fig:architecture}
\end{wrapfigure}

% In this section, we detail \snowy's design and implementation.
% As highlighted in Section~\ref{sec:scenario}, \snowy~is a multimodal system that supports natural language input as well as direct manipulation interactions through the graphical user interface (GUI).
Incorporating the aforementioned design considerations, we developed \snowy~as a \todo{prototype/design probe} to investigate the idea of leveraging NL utterance recommendations for guiding visual analysis while implicitly helping people discover and learn the system's NL capabilities.
In this section, we first briefly describe \snowy's interface and walk-through a usage scenario that exemplifies how NL utterance recommendations can aid conversational visual analysis.
We subsequently detail \snowy's design and implementation, discussing how it leverages a combination of features from the underlying data along with the users' interaction context to present in-situ utterance recommendations.


\input{sections/system/interface}

\subsection{System Overview}
% arjun: Depending on Vidya's initial reaction, add a couple of sentences about how having this combination provides an equivalent setup for prior systems with features like ambiguity and query refinement widgets.
\snowy~is implemented as a web-based application and is developed using Python, HTML/CSS, and JavaScript.
Visualizations in the tool are specified and created using Vega-Lite~\cite{satyanarayan2016vega}.
Figure~\ref{fig:architecture} presents a high-level depiction of the system's architecture.
There are three main components including the \textit{Interface Manager}, \textit{Natural Language Interpreter}, and the \textit{Utterance Recommendation Engine}.



\subsection{Interface Manager}
\label{sec:interface-manager}
\snowy is designed to be a context-sensitive recommendations interface that adapts an action-reaction design~\cite{}, where the user interaction causes the interface to react and update based on the actions that the user makes. Two types of contextual information are considered: explicit and implicit. Explicit user interactions are drag-and-drop-interactions, setting filters, typing of input NL queries, selection of recommendations, and the selection of one or marks in the visualization. Implicit interactions include data properties of the attributes involved in the various explicit interactions and syntactic structures of how users express their NL utterances in the interface.

The interface manager maintains the \textit{contextual state} of the interface; the information from both the explicit and implicit interactions that are used for generating natural language utterance recommendations.

\subsubsection{Modeling the context state}
The context state object is modeled as a combination of: 1) the active chart and mark selections, 2) the active utterance, and 3) the user's data exploration history.
The first two are directly captured from the visualization canvas (Figure~\ref{fig:teaser}D) and the input box (Figure~\ref{fig:teaser}C), respectively.
The data exploration history is stored as interaction scores corresponding to attributes, values, and the five analytic intents supported in \snowy~(distribution, correlation, derived value, trend, and filter).

For attributes and values, the interaction scores are computed by tracking the number of times data attributes been mapped to visual encodings or data values are applied as filters.
For intents, the scores are incremented in three scenarios.
First, when utterance recommendations are selected, the score for the recommendations' corresponding intent is incremented (e.g.~selecting the recommendation \reco{Show average \textbf{Worldwide Gross} by \textbf{Major Genre}} in Figure~\ref{fig:scenario-1}D increments the score for the \textit{derived value} intent).
Second, when natural language utterances are manually entered, scores corresponding to intents in the input utterances are incremented based on the output of the natural language interpreter (more details in the forthcoming Section~\ref{sec:nl-interpreter}).
And third, specifically for the filter intent, the score is also incremented if new filters are manually applied through the GUI.

\subsection{Natural Language Interpreter}
\label{sec:nl-interpreter}
\input{sections/system/parser}

\subsection{Utterance Recommendation Engine}
\label{sec:reco-engine}
\input{sections/system/reco}

==> sections/outline.tex <==
\section{Outline}

\begin{itemize}
    \item Intro
    \item RW
    \item Design Considerations
    \item System
    % general intro para
    % 1. scenario
    % 2. Architecture and components
    \item Study
    \item Discussion
    \item Future Work
    \item Conclusion
\end{itemize}

==> tables/intents.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{wraptable}{r}{0cm}
\centering
\resizebox{.525\textwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\vspace{.3em}
\intent{Distribution} & \begin{tabular}{@{}ll@{}}Observing the spread of values or number of items in a\\dataset with respect to a single attribute.\end{tabular}\\
\vspace{.3em}
\intent{Group} & \begin{tabular}{@{}ll@{}}Comparing values or groups within a categorical attribute\\with respect to a quantitative attribute.\end{tabular} \\
\vspace{.3em}
\intent{Correlation} & \begin{tabular}{@{}ll@{}}Understanding the effect of the change in one quantitative\\attribute to another quantitative attribute.\end{tabular} \\
\vspace{.3em}
\intent{Trend} & \begin{tabular}{@{}ll@{}}Observing the changes in values for a quantitative attribute\\over a temporal attribute.\end{tabular} \\
\vspace{.3em}
\intent{Filter} & \begin{tabular}{@{}ll@{}}Drill down into a subset of the data based on specific attributes\\and values.\end{tabular} \\
\intent{Aggregation} & \begin{tabular}{@{}ll@{}}Applying specific calculations (e.g., mean, sum) on a\\quantitative attribute over a categorical or temporal attribute.\end{tabular} \\\bottomrule
\end{tabular}%
}
\caption{Intents supported in current prototype along with a brief description of the analytic task that each intent maps to. Filter and aggregation are typically used as secondary tasks after or in conjunction with the first four.}
\vspace{-2em}
\label{tab:intents}
\end{wraptable}
